IC-World: In-Context Generation for Shared World Modeling

Video-based world models have recently garnered increasing attention for their ability to synthesize diverse and dynamic visual environments. In this paper, we focus on shared world modeling, where a model generates multiple videos from a set of input images, each representing the same underlying world in different camera poses. We propose IC-World, a novel generation framework, enabling parallel generation for all input images via activating the inherent in-context generation capability of large video models. We further finetune IC-World via reinforcement learning, Group Relative Policy Optimization, together with two proposed novel reward models to enforce scene-level geometry consistency and object-level motion consistency among the set of generated videos. Extensive experiments demonstrate that IC-World substantially outperforms state-of-the-art methods in both geometry and motion consistency. To the best of our knowledge, this is the first work to systematically explore the shared world modeling problem with video-based world models.

==> resources/tables/comparison_dynamic.tex <==
%%%%%%%%%%%%% 2023/07/25 update %%%%%%%%%%%%%

\begin{table*}[t]
    \centering
    \begin{adjustbox}{width=\linewidth}
        \begin{threeparttable}
            \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|}
            \hline
            Models & WorldScore-Static & WorldScore-Dynamic & Camera Ctrl & Object Ctrl & Content Align & 3D Consist & Photo Consist & Style Consist & Subjective Qual & Motion Acc & Motion Mag & Motion Smooth \\
            \hline
            Gen-3  & 60.71 & 57.58 & 59.24 & 50.49 & 69.56 & 73.53 & 87.09 & 62.82 & 63.85 & 54.53 & 27.48 & 68.87 \\
            Hailuo  & 57.55 & 56.36 & 29.47 & 62.92 & 69.56 & 73.53 & 67.18 & 87.09 & 62.82 & 63.85 & 64.76 & 70.07 \\
            \hline
            Wan2.1 & 57.56 & 52.85 & 23.53 & 40.32 & 45.44 & 78.74 & 78.36 & 77.18 & 59.38 & 54.27 & 33.26 & 38.05 \\
            DynamiCrafter  & 52.09 & 47.19 & 25.15 & 47.36 & 25.00 & 72.90 & 60.95 & 78.85 & 54.40 & 41.11 & 39.25 & 26.92 \\
            VideoCrafter1-T2V & 47.10 & 43.54 & 21.61 & 50.44 & 60.78 & 64.86 & 51.36 & 38.05 & 42.63 & 11.76 & 75.00 & 18.87 \\
            VideoCrafter1-I2V  & 50.47 & 47.64 & 25.21 & 52.24 & 73.89 & 64.90 & 56.77 & 43.79 & 56.74 & 47.12 & 30.40 & 29.39 \\
            VideoCrafter2  & 52.57 & 47.49 & 29.34 & 46.88 & 75.23 & 58.68 & 61.85 & 43.79 & 56.74 & 47.12 & 30.40 & 29.39 \\
            T2V-Turbo & 45.65 & 40.51 & 17.81 & 55.56 & 64.78 & 51.36 & 58.51 & 51.36 & 45.67 & 50.24 & 42.18 & 26.25 \\
            EasyAnimate & 52.85 & 51.65 & 26.72 & 54.76 & 64.60 & 62.92 & 55.53 & 42.46 & 44.67 & 27.62 & 60.16 & 37.09 \\
            CogVideoX-T2V & 54.18 & 48.79 & 29.84 & 62.81 & 68.81 & 64.20 & 42.19 & 41.67 & 25.00 & 69.66 & 25.06 & 60.15 \\
            CogVideoX-I2V  & 62.15 & 59.34 & 36.27 & 68.63 & 68.81 & 68.11 & 64.20 & 42.19 & 44.67 & 50.51 & 56.61 & 60.26 \\
            Allegro  & 55.31 & 51.84 & 29.87 & 64.70 & 71.12 & 58.68 & 57.02 & 42.30 & 51.46 & 31.87 & 37.22 & 35.43 \\
            Vchitect-2.0 & 42.28 & 38.48 & 26.55 & 49.54 & 65.75 & 41.53 & 42.30 & 25.69 & 44.58 & 33.59 & 33.81 & 21.31 \\
            \hline
            CogVideoX-I2V  & 62.15 & 59.34 & 36.27 & 68.63 & 68.81 & 68.11 & 64.20 & 42.19 & 44.67 & 50.51 & 56.61 & 60.26 \\
            CogVideoX-I2V + IC \\
            Hunyuan-Video \\
            Hunyuan-Video + IC \\
            Wan2.2-14B-distill & 62.46 & 57.19 & 31.36 & 38.87 & 55.29 & 77.77 & 86.26 & 85.3 & 62.38 & 56.95 & 26.48 & 51.20 \\
            Wan2.2-14B-distill + IC & \\
            \hline
            \end{tabular}
        \end{threeparttable}
    \end{adjustbox}
    \caption{Comparison of various video generation models across multiple metrics.}
    \label{tab:world_Score}
\end{table*}


==> resources/tables/comparison_static.tex <==
%%%%%%%%%%%%% 2023/07/25 update %%%%%%%%%%%%%

\begin{table*}[t]
    \centering
    \begin{adjustbox}{width=\linewidth}
        \begin{threeparttable}
            \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|}
            \hline
            Models & WorldScore-Static & WorldScore-Dynamic & Camera Ctrl & Object Ctrl & Content Align & 3D Consist & Photo Consist & Style Consist & Subjective Qual & Motion Acc & Motion Mag & Motion Smooth \\
            \hline
            Gen-3  & 60.71 & 57.58 & 59.24 & 50.49 & 69.56 & 73.53 & 87.09 & 62.82 & 63.85 & 54.53 & 27.48 & 68.87 \\
            Hailuo  & 57.55 & 56.36 & 29.47 & 62.92 & 69.56 & 73.53 & 67.18 & 87.09 & 62.82 & 63.85 & 64.76 & 70.07 \\
            \hline
            Wan2.1 & 57.56 & 52.85 & 23.53 & 40.32 & 45.44 & 78.74 & 78.36 & 77.18 & 59.38 & 54.27 & 33.26 & 38.05 \\
            DynamiCrafter  & 52.09 & 47.19 & 25.15 & 47.36 & 25.00 & 72.90 & 60.95 & 78.85 & 54.40 & 41.11 & 39.25 & 26.92 \\
            VideoCrafter1-T2V & 47.10 & 43.54 & 21.61 & 50.44 & 60.78 & 64.86 & 51.36 & 38.05 & 42.63 & 11.76 & 75.00 & 18.87 \\
            VideoCrafter1-I2V  & 50.47 & 47.64 & 25.21 & 52.24 & 73.89 & 64.90 & 56.77 & 43.79 & 56.74 & 47.12 & 30.40 & 29.39 \\
            VideoCrafter2  & 52.57 & 47.49 & 29.34 & 46.88 & 75.23 & 58.68 & 61.85 & 43.79 & 56.74 & 47.12 & 30.40 & 29.39 \\
            T2V-Turbo & 45.65 & 40.51 & 17.81 & 55.56 & 64.78 & 51.36 & 58.51 & 51.36 & 45.67 & 50.24 & 42.18 & 26.25 \\
            EasyAnimate & 52.85 & 51.65 & 26.72 & 54.76 & 64.60 & 62.92 & 55.53 & 42.46 & 44.67 & 27.62 & 60.16 & 37.09 \\
            CogVideoX-T2V & 54.18 & 48.79 & 29.84 & 62.81 & 68.81 & 64.20 & 42.19 & 41.67 & 25.00 & 69.66 & 25.06 & 60.15 \\
            CogVideoX-I2V  & 62.15 & 59.34 & 36.27 & 68.63 & 68.81 & 68.11 & 64.20 & 42.19 & 44.67 & 50.51 & 56.61 & 60.26 \\
            Allegro  & 55.31 & 51.84 & 29.87 & 64.70 & 71.12 & 58.68 & 57.02 & 42.30 & 51.46 & 31.87 & 37.22 & 35.43 \\
            Vchitect-2.0 & 42.28 & 38.48 & 26.55 & 49.54 & 65.75 & 41.53 & 42.30 & 25.69 & 44.58 & 33.59 & 33.81 & 21.31 \\
            \hline
            CogVideoX-I2V  & 62.15 & 59.34 & 36.27 & 68.63 & 68.81 & 68.11 & 64.20 & 42.19 & 44.67 & 50.51 & 56.61 & 60.26 \\
            CogVideoX-I2V + IC \\
            Hunyuan-Video \\
            Hunyuan-Video + IC \\
            Wan2.2-14B-distill & 62.46 & 57.19 & 31.36 & 38.87 & 55.29 & 77.77 & 86.26 & 85.3 & 62.38 & 56.95 & 26.48 & 51.20 \\
            Wan2.2-14B-distill + IC & \\
            \hline
            \end{tabular}
        \end{threeparttable}
    \end{adjustbox}
    \caption{Comparison of various video generation models across multiple metrics.}
    \label{tab:world_Score}
\end{table*}


==> resources/tables/user_study.tex <==
%%%%%%%%%%%%% 2023/07/25 update %%%%%%%%%%%%%

\begin{table*}[h]
    \centering
    \begin{adjustbox}{width=\linewidth}
        \begin{threeparttable}
            \begin{tabular}{l|ccc|cc}
            \toprule
            \multirow{2}{*}{Methods} & \multicolumn{3}{c|}{Static scene + Dynamic camera} & \multicolumn{2}{c}{Dynamic scene + Static camera} \\
            & Geometry Consist. & Camera Control & Visual Quality & Motion Consist. & Visual Quality \\
            \midrule
            CogVideoX-I2V-5B & 22.5\% & 18.8\% & 27.5\% & 20.0\% & 26.3\% \\
            Wan2.1*-14B  & 26.3\% & 28.8\% & 21.3\% & 28.8\% & 22.5\% \\
            LTX-Video-13B & 7.5\% & 17.5\% & 18.8\% & 17.5\% & 20.0\% \\
            \midrule
            \methodname & 43.6\% & 35.0\% & 32.5\% & 33.8\% & 31.3\% \\
            \bottomrule
            \end{tabular}
        \end{threeparttable}
    \end{adjustbox}
    \caption{\textbf{User study.} Wan2.1* denotes the distilled version~\cite{lightx2v}. Each number represents the win rate of the method on the specific metrics. All numbers are rounded to one decimal place.}
    \label{tab:user_study}
\end{table*}



==> resources/tables/world_score.tex <==
%%%%%%%%%%%%% 2023/07/25 update %%%%%%%%%%%%%

% \begin{table*}[t]
%     \centering
%     \begin{adjustbox}{width=\linewidth}
%         \begin{threeparttable}
%             \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|}
%             \hline
%             Models & WorldScore-Static & WorldScore-Dynamic & Camera Ctrl & Object Ctrl & Content Align & 3D Consist & Photo Consist & Style Consist & Subjective Qual & Motion Acc & Motion Mag & Motion Smooth \\
%             \hline
%             Gen-3  & 60.71 & 57.58 & 59.24 & 50.49 & 69.56 & 73.53 & 87.09 & 62.82 & 63.85 & 54.53 & 27.48 & 68.87 \\
%             Hailuo  & 57.55 & 56.36 & 29.47 & 62.92 & 69.56 & 73.53 & 67.18 & 87.09 & 62.82 & 63.85 & 64.76 & 70.07 \\
%             \hline
%             Wan2.1 & 57.56 & 52.85 & 23.53 & 40.32 & 45.44 & 78.74 & 78.36 & 77.18 & 59.38 & 54.27 & 33.26 & 38.05 \\
%             DynamiCrafter  & 52.09 & 47.19 & 25.15 & 47.36 & 25.00 & 72.90 & 60.95 & 78.85 & 54.40 & 41.11 & 39.25 & 26.92 \\
%             VideoCrafter1-T2V & 47.10 & 43.54 & 21.61 & 50.44 & 60.78 & 64.86 & 51.36 & 38.05 & 42.63 & 11.76 & 75.00 & 18.87 \\
%             VideoCrafter1-I2V  & 50.47 & 47.64 & 25.21 & 52.24 & 73.89 & 64.90 & 56.77 & 43.79 & 56.74 & 47.12 & 30.40 & 29.39 \\
%             VideoCrafter2  & 52.57 & 47.49 & 29.34 & 46.88 & 75.23 & 58.68 & 61.85 & 43.79 & 56.74 & 47.12 & 30.40 & 29.39 \\
%             T2V-Turbo & 45.65 & 40.51 & 17.81 & 55.56 & 64.78 & 51.36 & 58.51 & 51.36 & 45.67 & 50.24 & 42.18 & 26.25 \\
%             EasyAnimate & 52.85 & 51.65 & 26.72 & 54.76 & 64.60 & 62.92 & 55.53 & 42.46 & 44.67 & 27.62 & 60.16 & 37.09 \\
%             CogVideoX-T2V & 54.18 & 48.79 & 29.84 & 62.81 & 68.81 & 64.20 & 42.19 & 41.67 & 25.00 & 69.66 & 25.06 & 60.15 \\
%             CogVideoX-I2V  & 62.15 & 59.34 & 36.27 & 68.63 & 68.81 & 68.11 & 64.20 & 42.19 & 44.67 & 50.51 & 56.61 & 60.26 \\
%             Allegro  & 55.31 & 51.84 & 29.87 & 64.70 & 71.12 & 58.68 & 57.02 & 42.30 & 51.46 & 31.87 & 37.22 & 35.43 \\
%             Vchitect-2.0 & 42.28 & 38.48 & 26.55 & 49.54 & 65.75 & 41.53 & 42.30 & 25.69 & 44.58 & 33.59 & 33.81 & 21.31 \\
%             \hline
%             CogVideoX-I2V  & 62.15 & 59.34 & 36.27 & 68.63 & 68.81 & 68.11 & 64.20 & 42.19 & 44.67 & 50.51 & 56.61 & 60.26 \\
%             Hunyuan-Video \\
%             Wan2.2-14B-distill & 62.46 & 57.19 & 31.36 & 38.87 & 55.29 & 77.77 & 86.26 & 85.3 & 62.38 & 56.95 & 26.48 & 51.20 \\
%             Wan2.1-14B-distill-1x2 & 48.44 & 45.78 & 24.8 & 38.69 & 68.59 & 51.77 & 33.71 & 65.4 & 56.14 & 51.53 & 46.44 & 20.76 \\
%             \hline
%             CogVideoX-I2V \\
%             Wan2.1-Base & 48.44 & 45.78 & 24.80 & 38.69 & 68.59 & 51.77 & 33.71 & 65.40 & 56.14 & 51.53 & 46.44 & 20.76 \\
%             Wan2.1-Cam+Geo & 49.07 & 46.30 & 25.47 & 38.18 & 69.91 & 52.74 & 34.39 & 66.51 & 56.29 & 52.21 & 46.20 & 21.09 \\
%             \hline
%             \end{tabular}
%         \end{threeparttable}
%     \end{adjustbox}
%     \caption{Comparison of various video generation models across multiple metrics. split to 2 tables}
%     \label{tab:world_Score}
% \end{table*}


\begin{table*}[]
    \centering
    \begin{adjustbox}{width=\linewidth}
        \begin{threeparttable}
            \begin{tabular}{lcccccccccccc}
            \hline
            \multirow{3}{*}{Models} & \multicolumn{2}{c}{WorldScore} & \multicolumn{3}{c}{Controllability} & \multicolumn{4}{c}{Quality} & \multicolumn{3}{c}{Dynamics} \\
            & \multirow{2}{*}{Static} & \multirow{2}{*}{Dynamics} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Camera\\ Ctrl\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Object\\ Ctrl\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Content\\ Align\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}3D\\ Consist\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Photo\\ Consist\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Style\\ Consist\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Subjective\\ Qual\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Motion\\ Acc\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Motion\\ Mag\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Motion\\ Smooth\end{tabular}} \\
            \\
            \hline
            % Gen-3 & 60.71 & 57.58 & 59.24 & 50.49 & 69.56 & 73.53 & 87.09 & 62.82 & 63.85 & 54.53 & 27.48 & 68.87 \\
            % CogVideoX-I2V & 62.15 & 59.34 & 36.27 & 68.63 & 68.81 & 68.11 & 64.20 & 42.19 & 44.67 & 50.51 & 56.61 & 60.26 \\
            % EasyAnimate & 52.85 & 51.65 & 26.72 & 54.76 & 64.60 & 62.92 & 55.53 & 42.46 & 44.67 & 27.62 & 60.16 & 37.09 \\
            % Wan2.1 & 57.56 & 52.85 & 23.53 & 40.32 & 45.44 & 78.74 & 78.36 & 77.18 & 59.38 & 54.27 & 33.26 & 38.05 \\
            VideoCrafter-I2V  & 50.47 & 47.64 & 25.21 & 52.24 & 73.89 & 64.90 & 56.77 & 43.79 & 56.74 & 47.12 & 30.40 & 29.39 \\
            Allegro  & 55.31 & 51.84 & 29.87 & 64.70 & 71.12 & 58.68 & 57.02 & 42.30 & 51.46 & 31.87 & 37.22 & 35.43 \\
            Vchitect-2.0 & 42.28 & 38.48 & 26.55 & 49.54 & 65.75 & 41.53 & 42.30 & 25.69 & 44.58 & 33.59 & 33.81 & 21.31 \\
            \hline
            \methodname \\
            \hline
            % 1x2 grid \\
            % \hline
            % CogVideoX-I2V \\
            % Wan2.1-IC & 47.48 & 45.09 & 23.49 & 39.19 & 67.84 & 50.59 & 32.42 & 63.06 & 55.76 & 51.51 & 45.88 & 21.15 \\
            % Wan2.1-IC+GRPO & 47.70 & 45.27 & 23.51 & 38.91 & 68.52 & 51.04 & 32.75 & 63.36 & 55.78 & 51.81 & 45.67 & 21.32 \\
            % \hline
            \end{tabular}
        \end{threeparttable}
    \end{adjustbox}
    \caption{Comparison of various video generation models across multiple metrics. split to 2 tables}
    \label{tab:world_Score}
\end{table*}
